Antenna bandwidth engineering through time-varying resistance

Operational bandwidth of resonant circuits is limited by the resonator's size, which is known as the Chu limit. This limit restricts miniaturization of antennas, as the antenna bandwidth is inversely proportional to its size. Here, we propose slow time modulation of resistive elements to engineer bandwidth of small antennas. The temporal modulation of resistance induces virtual impedance that is fully controlled by the modulation parameters. We show how the virtual impedance can be used to optimize the frequency response of a resonant circuit, leading to enhanced matching at multiple frequencies simultaneously. We experimentally verify the proposed technique, demonstrating enhancement of radiation of a broadband modulated signal radiated by a small antenna.

==> Extra.tex <==
Assume having $M$ input frequencies and $N$ modulation frequencies, assuming the gaps between the input frequencies are not equal and each $ \omega_{k}$ couples only with $ \omega_{-k}$ through $\Delta \omega_{k}$, using the same analytical approximation we obtained above, we find that the impedance added at each frequency is
\begin{equation}
  Z_{n}^\text{m}=\frac{a_{-n}}{a_{n}}0.5mR_0e^{j(\theta_{-n}+\phi_{|n|}.\frac{n}{|n|}-\theta_{n})} 
  \label{Eq:equation6} 
\end{equation}


\section{Matching enhancement for AM}

Here we show how a circuit can be almost perfectly matched for more than one frequency at the same time using the slow load modulation developed in the previous section. Consider the amplitude modulated signals
\begin{equation}
   V_\text{AM}=\cos{(\omega_{0}t)}.[a_{c}+a_{\text{s}}\cos{(\frac{\Delta \omega}{2}t+\theta)}]
   \label{Eq:equation8} %the label lets you refer to the equation later
\end{equation}
connected to the time modulated load $R(t)=R_0+R_0m~ \Re(e^{j\phi_1} e^{j{\Delta \omega} t})$. In addition, the circuit also includes reactive elements that resonate at $\omega_{0}$, and as any resonator, for frequencies higher than $\omega_{0}$ the reactive elements add positive (inductive) reactance, and for frequencies lower than $\omega_{0}$ they add negative (capacitive) reactance. For simplicity, assume that the reactances appear at $\omega_{0}\pm \frac{\Delta \omega}{2}$ due to the dispersion of the reactive elements are equal in magnitude $|X_{-1}|=|X_{1}|$ but has opposite signs. To use the same notation as previously, $V_\text{AM}$ can be written as 
 \begin{equation}
\begin{aligned}
 V_\text{AM}= & \ a_c \cos{(\omega_{0}t)}\\
      & + a_{-1}\cos{(\omega_{-1}t+\theta_{-1})}\\
      & + a_{1}\cos{(\omega_{1}t+\theta_{1})}  \
\end{aligned}
\label{Eq:equation8} 
\end{equation}
Where $a_{-1}=a_{1}=0.5 a_c a_{\text{s}}$, $-\theta_{-1}=\theta_{1}=\theta$ and $\omega_{0}\pm \frac{\Delta \omega}{2}=\omega_{\pm 1}$. If we choose $\phi_1=2\theta+\frac{3\pi}{2}$, according to the analytical approximation, we get that $X_{\pm 1}^\text{m}=\mp 0.5 m R_0$. By choosing a value for $m$ that satisfies $0.5 m R_0=|X_{-1,1}|$, the circuit become perfectly matched at all three frequencies, as the reactances added due to modulation cancel the existent reactances coming from the dispersion of the reactive elements. Note that the modulation term also couple with $\omega_{0}$, but the resultant signals are not in our band of interest which is $\omega_{0}\pm \frac{\Delta \omega}{2}$, so we ignore them.
\begin{figure}[t]
	\centerline{\includegraphics[width=0.9\linewidth]{Fig. 3.PNG}}
	\caption{}
	\vspace{-10pt}
	\label{Fig:RL(t)C_circuit}
\end{figure}

As an example, assume the circuit has capacitance $C=5.07[\text{pF}]$ and inductance $L=5[\text{nH}]$ that resonate at $\omega_0=1\text{GHz}$. Also, we have $\omega_{-1}=0.9\text{GHz}$, $\omega_{1}=1.1\text{GHz}$, $\theta=0$, $R_0=100$, $X_{-1}=-6.6\Omega$ and $X_{1}=6\Omega$. As $|X_{-1}|\neq|X_{1}|$, we can take the average $|X|_{av}=6.3$, which results in $m=\frac{|X|_{av}}{0.5 R_0}=0.126$. Then, we get $X_{\pm 1}^\text{m}=\mp 6.3 \Omega$. According to our analytical solution, the total effective impedance of the modulated circuit at $\omega_1$ and $\omega_{-1}$ equals
\begin{equation}
   Z_{eff}^{\omega_{-1}}=R_0+jX_{-1}+jX^m_{-1}=100-j0.3\Omega
   \label{Eq:equation8} %the label lets you refer to the equation later
\end{equation}
\begin{equation}
   Z_{eff}^{\omega_1}=R_0+jX_1+jX^m_1=100-j0.3\Omega
   \label{Eq:equation8} %the label lets you refer to the equation later
\end{equation}
respectively. The numerical results give
\begin{equation}
  Z_{eff}^{\omega_{-1}}=99.6-j0.4\Omega
   \label{Eq:equation8} %the label lets you refer to the equation later
\end{equation}
\begin{equation}
   Z_{eff}^{\omega_{1}}=99.6-j0.2\Omega
   \label{Eq:equation8} %the label lets you refer to the equation later
\end{equation}
\begin{equation}
   Z_{eff}^{\omega_{0}}=99.2\Omega
   \label{Eq:equation8} %the label lets you refer to the equation later
\end{equation}
The reactance is mostly canceled at the side frequencies and no reactance is added at $\omega_0$. The input resistance is not exactly $100$ anymore, but the change in the resistance is not significant. In addition, decreasing the resistance means power amplification, which might be useful in some cases.  Again, as long as $\phi_1=2\theta+\frac{3\pi}{2}$, $Z_{\pm 1}^\text{m}$ does not depend on $\theta$, so it can vary in time without changing the modulation effect, which is shown in Fig. 3.

==> notes.tex <==
% At end of section 2 subsection B, clarify what is meant by gain and loss.

% Figure 2, y axes label, the t should be italic

% Figure 3 caption

% fix notations of the experimental sections to match the theoretical sections

% Revise

==> subsection_b_extra.tex <==
When an element is time varying, it adds different equivalent impedances at different frequencies. In this case, we need to define the effective impedance seen at each frequency. Similarly to [T-V circuits], the effective impedance at frequency $\omega_n$ can be defined as 
\begin{equation}
 Z^{\text{eff}}_{n}= \dfrac{\mathcal{F} [V(t)]\big|_{\omega=\omega_n}}{\mathcal{F}[I(t)]\big|_{\omega=\omega_n}}=Z^{\text{s}}_{n} + Z^{\text{m}}_{n} ,
   \label{eq:imp-def} 
\end{equation}
where $\mathcal{F}$ is the Fourier transform operator, $Z^{\text{s}}_{n}$ is the impedance of the static elements and $ Z^{\text{m}}_{n}$ is the equivalent impedance added by modulation.
{\bf Here you introduce new notations for the same thing. Now you have $Z_{eq}$ and $Z^m$ which mean the same. And there is also $Z^{eff}$. Please select only one notation and use it everywhere. I suggest $Z_n^{\rm eq}$ for the additional impedance at $\omega_n$ ("m" looks like the mth power).}

It is important to shed light on what is meant by the equivalent impedance seen at one specific frequency, and how is it different from a static impedance that produces the same current component (at the same frequency). Any static circuit element (e.g., a capacitor) has an effect at all input frequencies. In contrast, the equivalent impedance added due to modulation affects only one specific frequency. We call it \emph{equivalent impedance} as it contributes to the ratio between the voltage and current components at the corresponding frequency. As an example, assume the voltage source in Eq.~\eqref{eq:volsou1} the input voltage has one more input frequency component at the  frequency $\omega_2$, where $\omega_2 \neq \omega_{\pm 1} \pm \omega_m$. As the modulation function will not create coupling to oscillations at $\omega_2$, the modulation does not affect the voltage to current ratio at frequency $\omega_2$, which means that  no equivalent impedance is added at this frequency. However, there are additional equivalent impedances added at frequencies $\omega_{\pm 1}$. This example highlights an interesting possibility, where we can add different equivalent impedances at different frequencies and engineer the effective impedance. This possibility can have many applications, for example, it can be used to match a circuit at all input frequencies.
